Galerkin v. least-squares Petrov--Galerkin projection in nonlinear model reduction

Least-squares Petrov--Galerkin (LSPG) model-reduction techniques such as the Gauss--Newton with Approximated Tensors (GNAT) method have shown promise, as they have generated stable, accurate solutions for large-scale turbulent, compressible flow problems where standard Galerkin techniques have failed. However, there has been limited comparative analysis of the two approaches. This is due in part to difficulties arising from the fact that Galerkin techniques perform optimal projection associated with residual minimization at the time-continuous level, while LSPG techniques do so at the time-discrete level. This work provides a detailed theoretical and computational comparison of the two techniques for two common classes of time integrators: linear multistep schemes and Runge--Kutta schemes. We present a number of new findings, including conditions under which the LSPG ROM has a time-continuous representation, conditions under which the two techniques are equivalent, and time-discrete error bounds for the two approaches. Perhaps most surprisingly, we demonstrate both theoretically and computationally that decreasing the time step does not necessarily decrease the error for the LSPG ROM; instead, the time step should be `matched' to the spectral content of the reduced basis. In numerical experiments carried out on a turbulent compressible-flow problem with over one million unknowns, we show that increasing the time step to an intermediate value decreases both the error and the simulation time of the LSPG reduced-order model by an order of magnitude.

==> flowchart.tex <==
\newcommand{\myline}[2]{
\path(#1.south) --(#2.north)  coordinate[pos=0.4](mid);
\draw[-latex,black,very thick] (#1.south) -| (mid) -| (#2.north);
}
\newcommand{\mylineHoriz}[2]{
\path(#1.west) --(#2.east)  coordinate[pos=0.4](mid);
\draw[-latex,black,very thick] (#1.west) |- (mid) |- (#2.east);
}

 \begin{figure}[htbp]
  \centering
\scriptsize
\begin{center}

  \begin{tikzpicture} [node distance=.5cm, start chain=going below,inner sep=5pt]
   \node[punktchain, join, text width=9em,minimum height=0.5cm] (ODE) {Full-order model\\ ODE};
	\begin{scope}
	[start branch=pgCont going left]
		 \node[approxMeth,text width=7.5em,minimum height=0.5cm] (PgprojCont) {Petrov--Galerkin\\ projection};
		 \node[punktchaindash] (DiscOptROMODE) {\reviewerA{Least-squares\\
		 Petrov--Galerkin} ROM\\ ODE};
	\begin{scope}
	[start branch=discOptGo going below]
		 \node[approxMeth,text width=9em,minimum height=0.5cm] (discOptprojtd) {time discretization};
		 %\node[punktchain,join] (DiscOptROM) {Galerkin ROM\\ ODE};
	\end{scope}
	\end{scope}
	\begin{scope}
	[start branch=galCont going right]
		 \node[approxMeth,join, text width=5em,minimum height=0.5cm] (GalprojCont)
		 {Galerkin projection};
		 \node[optpunktchain,join] (DiscOptROM) {\reviewerA{Galerkin} ROM\\ ODE};

	\begin{scope}
	[start branch=galDiscGo going below]
		 \node[approxMeth,join, text width=9em,minimum height=0.5cm] (Galprojtd) {time discretization};
		 %\node[punktchain,join] (DiscOptROM) {Galerkin ROM\\ ODE};
	\end{scope}
	\end{scope}
   \node[approxMeth, join, text width=9em,minimum height=0.5cm] (FOMtd) {time discretization};
   \node[punktchain, join, text width=9em,minimum height=0.5cm] (ODeltaE) {Full-order model\\ O$\Delta$E};
	\begin{scope}
	[start branch=galDisc going right]
		 \node[approxMeth,join, text width=5em,minimum height=0.5cm] (Galproj) {Galerkin\\ projection};
		 \node[punktchain,join] (galODeltaE) {\reviewerA{Galerkin} ROM\\ O$\Delta$E};
	\end{scope}
	\begin{scope}
	[start branch=discopt going left]
		 \node[approxMeth,join, text width=7.5em,minimum height=0.5cm]
		 (optProjDisc) {\reviewerA{Petrov--Galerkin\\ projection}};
		 \node[optpunktchain,join] (DiscOptROM) {\reviewerA{Least-squares\\
		 Petrov--Galerkin} ROM\\ O$\Delta$E};
	%\begin{scope}
	%[start branch=discoptCont going above]
		 %\node[approxMeth,join, text width=9em,minimum height=0.5cm] (optProjDisc) {test subspace};
		 %\node[punktchain,join] (DiscOptROMODE) {Discrete-optimal ROM\\ ODE};
	%\end{scope}
	\end{scope}
\myline{Galprojtd}{galODeltaE}
%\myline{discOptprojtd}{DiscOptROM}
\path [line,dashed] (PgprojCont) -- (ODE);
\path [line,dashed] (DiscOptROMODE) -- (PgprojCont);
\path [line,dashed] (discOptprojtd) -- (DiscOptROMODE);
\path [line,dashed] (DiscOptROM) -- (discOptprojtd);
%\myline{discOptprojtd}{DiscOptROM}
  \end{tikzpicture}
  \end{center}
\caption{Relationship between Galerkin and discrete-optimal ROMs at the
time-continuous \reviewerB{(ODE)} and time-discrete \reviewerB{(O$\Delta$E)}
levels. Bolded outlines imply \reviewerA{the ROM associates with a minimum-residual
solution at that time-discretization level}.
Dashed lines imply the relationships are valid under certain conditions (see
Theorems \ref{thm:discOptROMcontDiscEqual} and
\ref{thm:discOptROMcontDiscEqualRK}).}
\label{fig:flowchart}
\end{figure}

